Force-Field-Enhanced Neural Network Interactions: from Local Equivariant Embedding to Atom-in-Molecule properties and long-range effects

We introduce FENNIX (Force-Field-Enhanced Neural Network InteraXions), a hybrid approach between machine-learning and force-fields. We leverage state-of-the-art equivariant neural networks to predict local energy contributions and multiple atom-in-molecule properties that are then used as geometry-dependent parameters for physically-motivated energy terms which account for long-range electrostatics and dispersion. Using high-accuracy ab initio data (small organic molecules/dimers), we trained a first version of the model. Exhibiting accurate gas-phase energy predictions, FENNIX is transferable to the condensed phase. It is able to produce stable Molecular Dynamics simulations, including nuclear quantum effects, for water predicting accurate liquid properties. The extrapolating power of the hybrid physically-driven machine learning FENNIX approach is exemplified by computing: i) the solvated alanine dipeptide free energy landscape; ii) the reactive dissociation of small molecules.

==> acronyms.tex <==
~\\
\section{List of abbreviations}
\begin{tabular}{ l l }
\printacr{adqtb}{adQTB}{Adaptive Quantum Thermal Bath}
\printacr{atcf}{ATCF}{Autocorrelation Function}
\printacr{cb}{CB}{Combination Band}
\printacr{cmd}{CMD}{Centroid Molecular Dynamics}
\printacr{dvr}{DVR}{Discrete Variable Representation}
\printacr{ecma}{ECMA}{Edgeworth Conditional Momentum Approximation}
\printacr{ir}{IR}{Infrared}
\printacr{ivr0}{IVR0}{Equilibrium Harmonic Approximation}
\printacr{lga}{LGA}{Local Gaussian Approximation}
\printacr{lha}{LHA}{Local Harmonic Approximation}
\printacr{lscivr}{LSC-IVR}{Linearized Semi-Classical Initial Value Representation}
\printacr{mctdh}{MCTDH}{Multi-Configuration Time-Dependent Hartree}
\printacr{md}{MD}{Molecular Dynamics}
\printacr{nqe}{NQE}{Nuclear Quantum Effect}
\printacr{pi}{PI}{Path Integral}
\printacr{pimd}{PIMD}{Path Integral Molecular Dynamics}
\printacr{qcmd}{QCMD}{Quasi-Centroid Molecular Dynamics}
\printacr{qtb}{QTB}{Quantum Thermal Bath}
\printacr{rpmd}{RPMD}{Ring-Polymer Molecular Dynamics}
\printacr{tcf}{TCF}{Time Correlation Function}
\printacr{trpmd}{TRPMD}{Thermostatted Ring-Polymer Molecular Dynamics}
\printacr{vdos}{VDOS}{Vibrational Density of States}
\printacr{wild}{WiLD}{Wigner-Langevin Dynamics}
\printacr{zpe}{ZPE}{Zero-Point Energy}
\printacr{zpel}{ZPEL}{Zero-Point Energy Leakage}
\end{tabular}
